Beyond Pairwise Comparisons in Social Choice: A Setwise Kemeny Aggregation Problem

In this paper, we advocate the use of setwise contests for aggregating a set of input rankings into an output ranking. We propose a generalization of the Kemeny rule where one minimizes the number of k-wise disagreements instead of pairwise disagreements (one counts 1 disagreement each time the top choice in a subset of alternatives of cardinality at most k differs between an input ranking and the output ranking). After an algorithmic study of this k-wise Kemeny aggregation problem, we introduce a k-wise counterpart of the majority graph. This graph reveals useful to divide the aggregation problem into several sub-problems, which enables to speed up the exact computation of a consensus ranking. By introducing a k-wise counterpart of the Spearman distance, we also provide a 2-approximation algorithm for the k-wise Kemeny aggregation problem. We conclude with numerical tests.

==> figApprox.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}

\definecolor{color0}{rgb}{1,0.498039215686275,0.0549019607843137}

\begin{groupplot}[group style={group size=3 by 1}]
\nextgroupplot[
tick align=outside,
tick pos=left,
title={\(\displaystyle \phi\!=\!\)0.65},
x grid style={white!69.0196078431373!black},
xlabel={value of \(\displaystyle k\)},
xmin=0.5, xmax=5.5,
xtick style={color=black},
xtick={1,2,3,4,5},
xticklabels={2,3,4,5,6},
y grid style={white!69.0196078431373!black},
ylabel={approximation ratio},
ymin=0.998, ymax=1.04,
ytick style={color=black},
ytick={0.995,1,1.005,1.01,1.015,1.02,1.025,1.03,1.035,1.04},
yticklabels={
  \(\displaystyle {0.995}\),
  \(\displaystyle {1.000}\),
  \(\displaystyle {1.005}\),
  \(\displaystyle {1.010}\),
  \(\displaystyle {1.015}\),
  \(\displaystyle {1.020}\),
  \(\displaystyle {1.025}\),
  \(\displaystyle {1.030}\),
  \(\displaystyle {1.035}\),
  \(\displaystyle {1.040}\)
}
]
\addplot [black]
table {%
0.75 1
1.25 1
1.25 1.00973929210071
0.75 1.00973929210071
0.75 1
};
\addplot [black]
table {%
1 1
1 1
};
\addplot [black]
table {%
1 1.00973929210071
1 1.01960784313725
};
\addplot [black]
table {%
0.875 1
1.125 1
};
\addplot [black]
table {%
0.875 1.01960784313725
1.125 1.01960784313725
};
\addplot [black]
table {%
1.75 1
2.25 1
2.25 1.00810630253752
1.75 1.00810630253752
1.75 1
};
\addplot [black]
table {%
2 1
2 1
};
\addplot [black]
table {%
2 1.00810630253752
2 1.01927194860814
};
\addplot [black]
table {%
1.875 1
2.125 1
};
\addplot [black]
table {%
1.875 1.01927194860814
2.125 1.01927194860814
};
\addplot [black, mark=o, mark size=3, mark options={solid,fill opacity=0}, only marks]
table {%
2 1.02185548617306
2 1.02047131635325
};
\addplot [black]
table {%
2.75 1
3.25 1
3.25 1.00636151559995
2.75 1.00636151559995
2.75 1
};
\addplot [black]
table {%
3 1
3 1
};
\addplot [black]
table {%
3 1.00636151559995
3 1.0128055878929
};
\addplot [black]
table {%
2.875 1
3.125 1
};
\addplot [black]
table {%
2.875 1.0128055878929
3.125 1.0128055878929
};
\addplot [black, mark=o, mark size=3, mark options={solid,fill opacity=0}, only marks]
table {%
3 1.01696410395603
3 1.02356970185334
3 1.01911145974471
3 1.01646549462083
3 1.01931855772412
};
\addplot [black]
table {%
3.75 1
4.25 1
4.25 1.00496738943534
3.75 1.00496738943534
3.75 1
};
\addplot [black]
table {%
4 1
4 1
};
\addplot [black]
table {%
4 1.00496738943534
4 1.01191301607312
};
\addplot [black]
table {%
3.875 1
4.125 1
};
\addplot [black]
table {%
3.875 1.01191301607312
4.125 1.01191301607312
};
\addplot [black, mark=o, mark size=3, mark options={solid,fill opacity=0}, only marks]
table {%
4 1.01644982317251
4 1.01607056549058
4 1.02384016849003
4 1.01730710113741
4 1.01471564186167
4 1.0177200236267
};
\addplot [black]
table {%
4.75 1
5.25 1
5.25 1.00357776805224
4.75 1.00357776805224
4.75 1
};
\addplot [black]
table {%
5 1
5 1
};
\addplot [black]
table {%
5 1.00357776805224
5 1.00738560743809
};
\addplot [black]
table {%
4.875 1
5.125 1
};
\addplot [black]
table {%
4.875 1.00738560743809
5.125 1.00738560743809
};
\addplot [black, mark=o, mark size=3, mark options={solid,fill opacity=0}, only marks]
table {%
5 1.01933045971555
5 1.0148134991119
5 1.02321341144295
5 1.01546753748376
5 1.0151372759616
5 1.01164398515392
5 1.01126530043703
5 1.0150251867292
};
\addplot [color0]
table {%
0.75 1.00522876710456
1.25 1.00522876710456
};
\addplot [color0]
table {%
1.75 1.00276225223827
2.25 1.00276225223827
};
\addplot [color0]
table {%
2.75 1.00208789230539
3.25 1.00208789230539
};
\addplot [color0]
table {%
3.75 1.00124605503969
4.25 1.00124605503969
};
\addplot [color0]
table {%
4.75 1.00074641780206
5.25 1.00074641780206
};

\nextgroupplot[
tick align=outside,
tick pos=left,
title={\(\displaystyle \phi\!=\!\)0.8},
x grid style={white!69.0196078431373!black},
xlabel={value of \(\displaystyle k\)},
xmin=0.5, xmax=5.5,
xtick style={color=black},
xtick={1,2,3,4,5},
xticklabels={2,3,4,5,6},
y grid style={white!69.0196078431373!black},
ylabel={approximation ratio},
ymin=0.998, ymax=1.04,
ytick style={color=black},
ytick={0.995,1,1.005,1.01,1.015,1.02,1.025,1.03,1.035,1.04},
yticklabels={
  \(\displaystyle {0.995}\),
  \(\displaystyle {1.000}\),
  \(\displaystyle {1.005}\),
  \(\displaystyle {1.010}\),
  \(\displaystyle {1.015}\),
  \(\displaystyle {1.020}\),
  \(\displaystyle {1.025}\),
  \(\displaystyle {1.030}\),
  \(\displaystyle {1.035}\),
  \(\displaystyle {1.040}\)
}
]
\addplot [black]
table {%
0.75 1.00380735605071
1.25 1.00380735605071
1.25 1.01746784933594
0.75 1.01746784933594
0.75 1.00380735605071
};
\addplot [black]
table {%
1 1.00380735605071
1 1
};
\addplot [black]
table {%
1 1.01746784933594
1 1.03153988868275
};
\addplot [black]
table {%
0.875 1
1.125 1
};
\addplot [black]
table {%
0.875 1.03153988868275
1.125 1.03153988868275
};
\addplot [black]
table {%
1.75 1.00333244417258
2.25 1.00333244417258
2.25 1.01358747823275
1.75 1.01358747823275
1.75 1.00333244417258
};
\addplot [black]
table {%
2 1.00333244417258
2 1.00032226877216
};
\addplot [black]
table {%
2 1.01358747823275
2 1.02815078466268
};
\addplot [black]
table {%
1.875 1.00032226877216
2.125 1.00032226877216
};
\addplot [black]
table {%
1.875 1.02815078466268
2.125 1.02815078466268
};
\addplot [black, mark=o, mark size=3, mark options={solid,fill opacity=0}, only marks]
table {%
2 1.03151774785802
2 1.03287487420329
};
\addplot [black]
table {%
2.75 1.00250131597438
3.25 1.00250131597438
3.25 1.01261295148296
2.75 1.01261295148296
2.75 1.00250131597438
};
\addplot [black]
table {%
3 1.00250131597438
3 1
};
\addplot [black]
table {%
3 1.01261295148296
3 1.02283883635612
};
\addplot [black]
table {%
2.875 1
3.125 1
};
\addplot [black]
table {%
2.875 1.02283883635612
3.125 1.02283883635612
};
\addplot [black, mark=o, mark size=3, mark options={solid,fill opacity=0}, only marks]
table {%
3 1.02865592494391
3 1.03137882535525
3 1.03463704795494
};
\addplot [black]
table {%
3.75 1.00175460948058
4.25 1.00175460948058
4.25 1.01187530861757
3.75 1.01187530861757
3.75 1.00175460948058
};
\addplot [black]
table {%
4 1.00175460948058
4 1
};
\addplot [black]
table {%
4 1.01187530861757
4 1.02659121753732
};
\addplot [black]
table {%
3.875 1
4.125 1
};
\addplot [black]
table {%
3.875 1.02659121753732
4.125 1.02659121753732
};
\addplot [black, mark=o, mark size=3, mark options={solid,fill opacity=0}, only marks]
table {%
4 1.02992271616355
4 1.03465146657167
};
\addplot [black]
table {%
4.75 1.00127771812579
5.25 1.00127771812579
5.25 1.01142994596372
4.75 1.01142994596372
4.75 1.00127771812579
};
\addplot [black]
table {%
5 1.00127771812579
5 1
};
\addplot [black]
table {%
5 1.01142994596372
5 1.02547536791709
};
\addplot [black]
table {%
4.875 1
5.125 1
};
\addplot [black]
table {%
4.875 1.02547536791709
5.125 1.02547536791709
};
\addplot [black, mark=o, mark size=3, mark options={solid,fill opacity=0}, only marks]
table {%
5 1.02708862978873
5 1.02690817715422
5 1.03376031721481
};
\addplot [color0]
table {%
0.75 1.00845879591224
1.25 1.00845879591224
};
\addplot [color0]
table {%
1.75 1.00658084539116
2.25 1.00658084539116
};
\addplot [color0]
table {%
2.75 1.00508631992606
3.25 1.00508631992606
};
\addplot [color0]
table {%
3.75 1.0046559474255
4.25 1.0046559474255
};
\addplot [color0]
table {%
4.75 1.00441336234909
5.25 1.00441336234909
};

\nextgroupplot[
tick align=outside,
tick pos=left,
title={\(\displaystyle \phi\!=\!\)0.95},
x grid style={white!69.0196078431373!black},
xlabel={value of \(\displaystyle k\)},
xmin=0.5, xmax=5.5,
xtick style={color=black},
xtick={1,2,3,4,5},
xticklabels={2,3,4,5,6},
y grid style={white!69.0196078431373!black},
ylabel={approximation ratio},
ymin=0.998, ymax=1.04,
ytick style={color=black},
ytick={0.995,1,1.005,1.01,1.015,1.02,1.025,1.03,1.035,1.04},
yticklabels={
  \(\displaystyle {0.995}\),
  \(\displaystyle {1.000}\),
  \(\displaystyle {1.005}\),
  \(\displaystyle {1.010}\),
  \(\displaystyle {1.015}\),
  \(\displaystyle {1.020}\),
  \(\displaystyle {1.025}\),
  \(\displaystyle {1.030}\),
  \(\displaystyle {1.035}\),
  \(\displaystyle {1.040}\)
}
]
\addplot [black]
table {%
0.75 1.01437343269803
1.25 1.01437343269803
1.25 1.02675585532902
0.75 1.02675585532902
0.75 1.01437343269803
};
\addplot [black]
table {%
1 1.01437343269803
1 1.00279916025192
};
\addplot [black]
table {%
1 1.02675585532902
1 1.03827072997874
};
\addplot [black]
table {%
0.875 1.00279916025192
1.125 1.00279916025192
};
\addplot [black]
table {%
0.875 1.03827072997874
1.125 1.03827072997874
};
\addplot [black]
table {%
1.75 1.008730937459
2.25 1.008730937459
2.25 1.019128306157
1.75 1.019128306157
1.75 1.008730937459
};
\addplot [black]
table {%
2 1.008730937459
2 1.00189178963299
};
\addplot [black]
table {%
2 1.019128306157
2 1.03080659593506
};
\addplot [black]
table {%
1.875 1.00189178963299
2.125 1.00189178963299
};
\addplot [black]
table {%
1.875 1.03080659593506
2.125 1.03080659593506
};
\addplot [black]
table {%
2.75 1.00674597171581
3.25 1.00674597171581
3.25 1.016004577127
2.75 1.016004577127
2.75 1.00674597171581
};
\addplot [black]
table {%
3 1.00674597171581
3 1.00101436338554
};
\addplot [black]
table {%
3 1.016004577127
3 1.02849186811413
};
\addplot [black]
table {%
2.875 1.00101436338554
3.125 1.00101436338554
};
\addplot [black]
table {%
2.875 1.02849186811413
3.125 1.02849186811413
};
\addplot [black]
table {%
3.75 1.0062306981514
4.25 1.0062306981514
4.25 1.01445398264171
3.75 1.01445398264171
3.75 1.0062306981514
};
\addplot [black]
table {%
4 1.0062306981514
4 1.00192364604913
};
\addplot [black]
table {%
4 1.01445398264171
4 1.02593855332998
};
\addplot [black]
table {%
3.875 1.00192364604913
4.125 1.00192364604913
};
\addplot [black]
table {%
3.875 1.02593855332998
4.125 1.02593855332998
};
\addplot [black]
table {%
4.75 1.00394035346418
5.25 1.00394035346418
5.25 1.01252522336342
4.75 1.01252522336342
4.75 1.00394035346418
};
\addplot [black]
table {%
5 1.00394035346418
5 1.00151181030759
};
\addplot [black]
table {%
5 1.01252522336342
5 1.02293837985402
};
\addplot [black]
table {%
4.875 1.00151181030759
5.125 1.00151181030759
};
\addplot [black]
table {%
4.875 1.02293837985402
5.125 1.02293837985402
};
\addplot [black, mark=o, mark size=3, mark options={solid,fill opacity=0}, only marks]
table {%
5 1.02574310598454
};
\addplot [color0]
table {%
0.75 1.01909012128479
1.25 1.01909012128479
};
\addplot [color0]
table {%
1.75 1.01389605103932
2.25 1.01389605103932
};
\addplot [color0]
table {%
2.75 1.01017285391194
3.25 1.01017285391194
};
\addplot [color0]
table {%
3.75 1.01014649693662
4.25 1.01014649693662
};
\addplot [color0]
table {%
4.75 1.00784598200297
5.25 1.00784598200297
};
\end{groupplot}

\end{tikzpicture}

